The Spectre of Surveillance and Censorship in Future Internet Architectures

Recent initiatives known as Future Internet Architectures (FIAs) seek to redesign the Internet to improve performance, scalability, and security. However, some governments perceive Internet access as a threat to their political standing and engage in widespread network surveillance and censorship. In this paper, we provide an in-depth analysis of the design principles of prominent FIAs in terms of their packet structure, addressing and naming schemes, and routing protocols to foster discussion on how these new systems interact with censorship and surveillance apparatuses. Further, we assess the extent to which existing surveillance and censorship mechanisms can successfully target FIA users while discussing privacy enhancing technologies to counter these mechanisms. We conclude by providing guidelines for future research into novel FIA-based privacy-enhancing technologies, and recommendations to guide the evaluation of these technologies.

==> sections/literature.tex <==
\section{Other Surveys on FIAs}
\label{sec:related_work}

A significant body of existing work has compared and contrasted different design aspects of FIAs~\cite{DBLP:journals/cm/PanPJ11,DBLP:journals/ieicet/Hasegawa13,DBLP:journals/ccr/Fisher14,DBLP:journals/access/DingYD16,mohammed2023future}. We rely on a similar understanding of the fundamental architectural elements of FIAs to facilitate our reasoning on the factors involved in routing traffic within FIAs.

Past research has surveyed the novel capabilities of different FIAs from a security and privacy perspective~\cite{DBLP:journals/comsur/AmbrosinCCGT18,lutzSecurity,DBLP:conf/imis/KhondokerNMB14}. Among these, we highlight extensive efforts at surveying security properties of content-centric networks~\cite{DBLP:journals/comsur/TouraniMMP18,DBLP:conf/lanman/GastiT18}, and NDN in particular~\cite{DBLP:journals/jcst/KumarSAS19, DBLP:journals/access/ShahLAB23, DBLP:journals/computers/HidouriHTHM22, DBLP:journals/corr/ChenM15f}. Unfortunately, a prevailing trend across much of this research is the examination of FIA designs' ability to address broader security threats such as denial of service, cache security, or intrusion detection. Notably, very little attention is paid to the susceptibility of FIA users' to surveillance and censorship efforts put forward by powerful network adversaries. Our survey aims to fill this gap by providing a comprehensive analysis of FIAs' resistance to surveillance and censorship efforts, and envisioning further improvements for potential FIA users' privacy.
